Properties of a family of n reggeized gluon states in multicolour QCD

A general relation between families of (n+1) gluon and n gluon eigenstates of the BKP evolution kernels in the multicolour limit of QCD is derived. It allows to construct an (n+1) gluon eigenstate if an n gluon eigenstate is known; this solution is Bose symmetric and thus physical for even n. A recently found family of odderon solutions corresponds to the particular case n=2.

==> fig1 <==
#FIG 3.2
Landscape
Center
Metric
A4      
50.00
Single
-2
1200 2
1 1 0 1 0 7 100 0 -1 0.000 1 0.0000 3375 1800 675 450 3375 1800 4050 2250
1 1 0 1 0 7 100 0 -1 0.000 1 0.0000 3375 3375 675 450 3375 3375 4050 3825
1 1 0 1 0 7 100 0 -1 0.000 1 0.0000 3375 4950 675 450 3375 4950 4050 5400
1 1 0 1 0 7 100 0 -1 0.000 1 0.0000 6525 1800 675 450 6525 1800 7200 2250
1 1 0 1 0 7 100 0 -1 0.000 1 0.0000 6525 4950 675 450 6525 4950 7200 5400
1 1 0 1 0 7 100 0 45 0.000 1 0.0000 3600 3195 270 180 3600 3195 3870 3375
1 1 0 1 0 7 100 0 45 0.000 1 0.0000 6300 4770 270 180 6300 4770 6570 4950
1 1 0 1 0 7 100 0 -1 0.000 1 0.0000 3375 6750 675 450 3375 6750 4050 7200
1 1 0 1 0 7 100 0 45 0.000 1 0.0000 3600 6570 270 180 3600 6570 3870 6750
2 1 0 2 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	3 1 2.00 90.00 180.00
	 6300 1800 3600 3150
2 1 0 2 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	3 1 2.00 90.00 180.00
	 3375 3600 6300 4725
2 1 0 2 0 7 100 0 -1 0.000 0 0 -1 1 0 2
	3 1 2.00 90.00 180.00
	 6300 5175 3600 6570
4 0 0 100 0 0 12 0.0000 7 165 270 1125 1800 $2$\001
4 0 0 100 0 0 12 0.0000 7 165 270 1125 3375 $3$\001
4 0 0 100 0 0 12 0.0000 7 165 270 1125 4950 $4$\001
4 0 0 100 0 0 12 0.0000 7 165 270 1125 6750 $5$\001
4 0 0 100 0 0 12 0.0000 7 165 270 1125 675 $n$\001
4 0 0 100 0 0 12 0.0000 7 195 870 2700 900 ($r_n=+1$)\001
4 0 0 100 0 0 12 0.0000 7 195 870 5850 900 ($r_n=-1$)\001
4 0 0 100 0 0 12 0.0000 7 135 1125 2475 540 EVEN STATE\001
4 0 0 100 0 0 12 0.0000 7 135 1020 5625 540 ODD STATE\001
4 0 0 100 0 0 20 0.0000 7 30 60 1215 8325 .\001
4 0 0 100 0 0 20 0.0000 7 30 60 1215 8775 .\001
4 0 0 100 0 0 20 0.0000 7 30 60 1215 9225 .\001
4 0 0 100 0 0 20 0.0000 7 30 60 4950 8325 .\001
4 0 0 100 0 0 20 0.0000 7 30 60 4950 8775 .\001
4 0 0 100 0 0 20 0.0000 7 30 60 4950 9225 .\001

